LSTM Fully Convolutional Networks for Time Series Classification

Fully convolutional neural networks (FCN) have been shown to achieve state-of-the-art performance on the task of classifying time series sequences. We propose the augmentation of fully convolutional networks with long short term memory recurrent neural network (LSTM RNN) sub-modules for time series classification. Our proposed models significantly enhance the performance of fully convolutional networks with a nominal increase in model size and require minimal preprocessing of the dataset. The proposed Long Short Term Memory Fully Convolutional Network (LSTM-FCN) achieves state-of-the-art performance compared to others. We also explore the usage of attention mechanism to improve time series classification with the Attention Long Short Term Memory Fully Convolutional Network (ALSTM-FCN). Utilization of the attention mechanism allows one to visualize the decision process of the LSTM cell. Furthermore, we propose fine-tuning as a method to enhance the performance of trained models. An overall analysis of the performance of our model is provided and compared to other techniques.

==> introduction-old.tex <==
Over the past decade, there has been an increased interest in time series classification and clustering. Time series data is ubiquitous, existing in weather readings, financial recordings, industrial observations, and psychological signals \cite{Wang_2017}. In this paper two deep learning models to classify time series datasets are proposed, both of which outperform existing state-of-the-art models.

Recently, deep learning approaches have been employed with time series classification algorithms. Multi-scale CNN (MCNN) \cite{cui2016multi}, fully convolutional network (FCN) \cite{wang2017time}, and residual network (ResNet) \cite{wang2017time} are deep learning approaches that take advantage of convolutional neural networks (CNN) for end-to-end classification of univariate time series. MCNN uses down-sampling, skip sampling and sliding window to preprocess the data. The classifier is highly dependent on the preprocessing and the large set of hyperparameters. On the other hand, FCN and ResNet do not require any heavy pre-processing on the data or feature crafting. In this paper, we improve the performance of FCN by concatenating CNN with a Long Term Short Term (LSTM) layer, LSTMFCN, or a LSTM layer with attention, ALSTMFCN. Similar to FCN, both proposed models can develop a Class Activation Maps (CAM) on the convolutional layers to detect regions that contribute to the class label more than others. In addition, the Attention LSTM layer can also be used detect regions that contribute to the class label through its VISUALS. Results indicate the new proposed models, LSTMFCN and ALSTMFCN, dramatically improve performance on the University of California Riverside (UCR) Benchmark datasets \cite{UCRArchive}.  

A plethora of research have been done using feature-based approaches or methods to extract a set of features that represent time series patterns. Bag-of-Words (BoW) \cite{Lin_2007}, Bag-of-features (TSBF) \cite{Baydogan_2013}, Bag-of-SFA-Symbols (BOSS) \cite{Sch_fer_2014}, BOSSVS \cite{schafer2016scalable}, Word ExtrAction for time SEries cLassification (WEASEL) \cite{Schafer_2017}, have obtained promising results in the field. Bag-of-words quantizes the extracted features and feeds the BoW into a classifier. TSBF extracts multiple subsequences of random local information, which a supervised learner condenses into a cookbook used to predict time series labels. BOSS introduces a combination of a distance based classifier and histograms. The histograms represent substructures of a time series that are created using a symbolic Fourier approximation. BOSSVS extends this method by proposing a vector space model to reduce time complexity while maintaining performance.  WEASEL converts time series into feature vectors using a sliding window. Machine learning algorithms utilize these feature vectors to detect and classify the time series.  All these classifiers require heavy feature extraction and feature crafting. One of the major advantages of LSTMFCN and ALSTMFCN is it does not require heavy preprocessing or feature crafting.

Ensemble algorithms also yield state-of-the-art performance with time series classification problems. Three of the most successful ensemble algorithms that integrate various features of a time series are Elastic Ensemble (PROP) \cite{Lines_2014}, a model that integrates 11 time series classifiers using a weighted ensemble method, Shapelet ensemble (SE) \cite{Bagnall_2016a}, a model that applies a heterogeneous ensemble onto transformed “shapelets”, and a flat collective of transform based ensembles (COTE) \cite{bagnall2015time}, a model that fuses 35 various classifiers into 1 classifier. LSTMFCN and ALSTMFCN produce better results than the Ensemble algorithms on a majority of the UCR Benchmark datasets. 

This paper proposes two deep learning models for end-to-end time series classification. The proposed models do not require heavy pre-processing on the data or feature crafting. Both the models are tested on all 85 UCR time series benchmarks and outperforms most of the state-of-the-art models. The remainder of the paper is organized as follows. Section \ref{Background Works} reviews the background work. Section \ref{LSTMFCN} presents the architecture of the proposed models. Section \ref{Experiments} analyzes and discusses theour experiments performed. Finally, we draw conclusions are drawn in Section \ref{conclusion}. 



==> old_introduction.tex <==
% In the past decade, there has been an increased interest in time series classification and clustering. Time series data is ubiquitous. It can be found everywhere, from human activities to nature. Some areas where time series data exists exist are in weather readings, financial recordings, industrial observations, and psychological signals (Wang 2017). Time series classification vary slightly from traditional classification techniques \cite{Bagnall_2016}. This is mainly due to the fact that time attributes are ordered. The objective of our paper is to develop a classifier that outperforms most of the current state of the art algorithms. 

% \par One of the earliest approaches for time series classification were distance-based methods, such as Euclidean Distance and Dynamic Time Warping (DTW)\cite{Keogh_2002}, combined with k-nearest neighbor classifiers. Subsequently, a plethora of research have been done using feature-based approaches or methods to extract a set of features that represent time series patterns. One of the most common feature-based technique, Bag-of-Words (BoW) \cite{Lin_2007}, quantizes the extracted features and feeds the BoW into a classifier. Other feature-based classifiers, the bag-of-features (TSBF) \cite{Baydogan_2013}, Bag-of-SFA-Symbols (BOSS) \cite{Sch_fer_2014}, BOSSVS \cite{Sch_fer_2015}, Word ExtrAction for time SEries cLassification (WEASEL) \cite{Schafer_2017}, have obtained promising results in the field. TSBF selects multiple subsequences of random length from random locations and extracts local information. With the use of a supervised learner, the local information is condensed into a cookbook that predicts the time series label. BOSS introduces a combination of a distance based classifier and histograms. The histograms represent substructures of a time series that are created using a symbolic Fourier approximation. BOSSVS extends this method by proposing a vector space model to reduce time complexity while maintaining performance. WEASEL is an scalable and accurate approach that converts time series into feature vectors using a  sliding window. Machine learning algorithms utilize these feature vectors to detect classify the time series.

% \par Ensemble algorithms have also been applied on time series problems. Three of the most successful ensemble algorithms, Elastic Ensemble (PROP) \cite{Lines_2014}, Shapelet ensemble (SE)\cite{Bagnall_2016a}, and a flat collective of transform based ensembles (COTE) \cite{Bagnall_2016a}, integrate various features with classifiers. PROP incorporates 11 time series classifiers through a weighted ensemble method. SE applies a heterogeneous ensemble onto transformed shapelets, a subsequence of a time series. COTE fuses 35 various classifiers, some of which extracts features from the time and frequency domain, into one classifier.

% \par More recently, deep learning approaches have been employed onto time series classification algorithms. Multi-channel convolutional neural network(MC-CNN), multi-scale CNN (MCNN), fully convolutional network (FCN), and residual network (ResNet) are favorable deep learning approaches that takes advantage of convolutional neural networks (CNN) for end-to-end classification. MC-CNN has been applied on multivariate time series classification (TSC) problems. In MC-CNN, the authors utilize sliding windows to enhance the data on each channel. The filters are applied on each channel. Subsequently, the outputs of each channel are then combined into a fully connected layer, which classifies the (TSC). MC-CNN has been applied onto two datasets, which are not made public. On the other hand, MCNN is tested on 44 benchmark time series datasets.  MCNN, a univariate time series classifier, uses down-sampling, skip sampling and sliding window to preprocess the data. The classifier is highly dependent on the preprocessing and the large set of hyper parameters. On the other hand, FCN and ResNet do not require any heavy pre-processing on the data or feature crafting. Yet, both FCN and ResNet achieve performance comparable to other state-of-the art methods.  
 
% \par In this paper, we propose two deep learning architecture, for end-to-end time series classification. Our proposed methods do not require heavy pre-processing on the data or feature crafting. Both our methods are tested on all 85 UCR time series benchmarks and outperforms most of the state of the art algorithms. The proposed architectures are similar to FCN, with an additional LSTM branch, that drastically improves performance. One of our architectures utilizes attention models, which helps detect important input sequences to the LSTM. In addition, we can develop Class Activation Maps (CAM) on the convolutional model to detect regions that contribute to the class label more than others.  
 
% \par The remainder of the paper is organized as follows. Section 2 reviews the related work. Section 3 presents the architecture of the proposed models. Section 4 analyzes and discusses our experiments. Finally, we draw conclusion in Section 5.  
